Lightweight Attentional Feature Fusion: A New Baseline for Text-to-Video Retrieval

In this paper we revisit feature fusion, an old-fashioned topic, in the new context of text-to-video retrieval. Different from previous research that considers feature fusion only at one end, let it be video or text, we aim for feature fusion for both ends within a unified framework. We hypothesize that optimizing the convex combination of the features is preferred to modeling their correlations by computationally heavy multi-head self attention. We propose Lightweight Attentional Feature Fusion (LAFF). LAFF performs feature fusion at both early and late stages and at both video and text ends, making it a powerful method for exploiting diverse (off-the-shelf) features. The interpretability of LAFF can be used for feature selection. Extensive experiments on five public benchmark sets (MSR-VTT, MSVD, TGIF, VATEX and TRECVID AVS 2016-2020) justify LAFF as a new baseline for text-to-video retrieval.

==> 4a.1.features.tex <==

%\subsubsection{Video / Text Features}
Eight video features and five text features are used, see \cref{tab:feature_intro}.
\input{table/feature_intro.tex}

==> fig/Fig_model_adjust_txt_vis_encoder.tex <==
% \begin{figure}
%   \centering
%   \begin{minipage}[]{0.48\linewidth} 
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=1\columnwidth]{Figure/model_adjust_txt_encoder.pdf} 
%     {{\small (a) Text feature fusion, with \{\emph{rx101},\emph{re152}\} as video features.}}
%     \label{fig:model_adjust_txt_encoder}
%   \end{minipage} 
% %   \hfill
%   \begin{minipage}[]{0.48\linewidth} 
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=1\columnwidth]{Figure/model_adjust_vis_encoder.pdf} 
%     {{\small (b) Video feature fusion, with \{\textit{bow,w2v,gru}\} as text features.}}
%     \label{fig:model_adjust_vis_encoder}
%     \end{minipage} 
%   \caption{\textbf{Performance curves of three distinct models, \ie W2VV++, SEA and the proposed LAFF}, with respect to (a) text feature fusion and (b) video feature fusion, respectively. LAFF is both effective and stable for fusing diverse features. Dataset: MSR-VTT-test3k.}
%   \label{fig:model_adjust_txt_vis_encoder}
%   \label{Figure:model_adjust_txt_vis_encoder}
% \end{figure}



\begin{figure}[htp]
\sbox\twosubbox{%
  \resizebox{\dimexpr\textwidth-1em}{!}{%
    \includegraphics[height=3cm]{Figure/model_adjust_txt_encoder.pdf} % \hspace
    \includegraphics[height=3cm]{Figure/model_adjust_vis_encoder.pdf}%
  }%
}
\setlength{\twosubht}{\ht\twosubbox}

\centering

\subcaptionbox{\label{fig:model_adjust_txt_encoder} Text feature fusion}{%
  \includegraphics[height=\twosubht]{Figure/model_adjust_txt_encoder.pdf}%
}\quad
\subcaptionbox{\label{fig:model_adjust_vis_encoder} Video feature fusion}{%
  \includegraphics[height=\twosubht]{Figure/model_adjust_vis_encoder.pdf}%
}
\caption{\textbf{Performance curves of three distinct models, \ie W2VV++, SEA and LAFF}, \wrt (a) text feature fusion, with \{\emph{rx101},\emph{re152}\} as video features, and (b) video feature fusion, with   \{\textit{bow,w2v,gru}\} as text features. LAFF is both effective and stable for fusing diverse features. Data: MV-test3k.}

  \label{Figure:model_adjust_txt_vis_encoder}

\end{figure}




==> fig/Fig_overall_framework.tex <==

\begin{figure}[htbp!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=1.0\textwidth]{Figure/overall_network.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\textbf{Conceptual diagram of using paired LAFF blocks for text-to-video retrieval}. Given a specific video $x$, we employ multiple (pre-trained) feature extractors to obtain a set of $k_1$ video-level features $\{f_{v,1}(x),\ldots,f_{v,k_1}(x)\}$. In a similar manner we extract from a query sentence $q$ a set of $k_2$ sentence-level features  $\{f_{t,1}(q),\ldots,f_{t,k_2}(q)\}$. Each pair of LAFFs determines a common space. In particular, a specific pair of LAFFs, indexed by $i$, aggregates the video (sentence) features into a $d$-dimensional cross-modal feature $e_i(x)$ ($e_i(q)$), and consequently computes the video-text similarity $s_i(x,q)$ per space. The sum of the similarities from all $h$ common spaces, \ie $\sum_{i=1}^h s_i(x,q)$, is used for retrieval.} %最终文档中希望显示的图片标题
\label{Figure:overall_framework} %用于文内引用的标签
\end{figure}

==> fig_multi_level_laff.tex <==
\begin{figure}[tb!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形

\begin{minipage}[b]{1\linewidth} %
\centering %图片居中
\includegraphics[width=0.7\textwidth]{Figure/LAFF_multi_level.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\rebuttal{\textbf{LAFF-ml for multi-level video feature fusion}}. }  %最终文档中希望显示的图片标题
\label{fig:LAFF_multi_level} %用于文内引用的标签
\end{minipage}%

\end{figure}

==> table/TV20_case_study.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[thp!]
\normalsize
\renewcommand\arraystretch{1}
\centering
\caption{\textbf{Performance of LAFF, CLIP-FT and CLIP2Video on TV20.} For CLIP-FT and CLIP2Video, no color font means the difference between infAP and LAFF is no more than 0.1, red font means infAP exceeds LAFF, and blue font means infAP is lower than LAFF.}
\label{tab:TV20_case_study}
\scalebox{0.6}{
% \arrayrulecolor{red}
\setlength{\tabcolsep}{2mm}{

\begin{tabular}{@{}lccccrrr@{}}
\toprule
\textbf{Query} & \textbf{Object} & \textbf{Person} & \textbf{Action} & \textbf{Location} & \textbf{LAFF} & \textbf{CLIP-FT} & \textbf{CLIP2Video} \\ \midrule 
641 showing an aerial view of   buildings near water in the daytime & \checkmark &  &  & \checkmark & 0.234 & 0.297 & 0.240 \\
642  a person paddling   kayak in the water & \checkmark & \checkmark & \checkmark & \checkmark & 0.430 & 0.399 & 0.445 \\
643  people dancing or   singing while wearing costumes outdoors &  & \checkmark & \checkmark &  & 0.134 & 0.080 & 0.071 \\
644  sailboats in the   water & \checkmark &  &  & \checkmark & 0.352 & {\color[HTML]{FF4343} 0.649} & {\color[HTML]{FF4343} 0.643} \\
645  a person wearing a   necklace & \checkmark & \checkmark &  &  & 0.034 & 0.036 & 0.088 \\
646  a woman sitting on   the floor & \checkmark & \checkmark &  &  & 0.163 & 0.091 & 0.106 \\
647  people or cars   moving on a dirt road & \checkmark & \checkmark & \checkmark &  & 0.267 & 0.199 & 0.223 \\
648  a man in blue jeans   outdoors & \checkmark & \checkmark &  & \checkmark & 0.053 & 0.018 & 0.081 \\
649  someone jumping   while snowboarding &  & \checkmark & \checkmark &  & 0.785 & {\color[HTML]{21A0FF} 0.448} & {\color[HTML]{21A0FF} 0.451} \\
650  one or more people   drinking wine &  & \checkmark & \checkmark &  & 0.096 & 0.054 & 0.040 \\
651  one or more people   skydiving &  & \checkmark & \checkmark &  & 0.489 & {\color[HTML]{21A0FF} 0.352} & 0.427 \\
652  a little boy smiling &  & \checkmark & \checkmark &  & 0.165 & 0.197 & 0.203 \\
653  group of people   clapping &  & \checkmark & \checkmark &  & 0.349 & {\color[HTML]{21A0FF} 0.082} & {\color[HTML]{21A0FF} 0.120} \\
654  one or more persons   exercising in a gym &  & \checkmark & \checkmark & \checkmark & 0.253 & 0.227 & 0.179 \\
655  one or more persons   standing in a body of water &  & \checkmark & \checkmark & \checkmark & 0.023 & 0.018 & 0.031 \\
656  a long haired man & \checkmark & \checkmark &  &  & 0.400 & {\color[HTML]{21A0FF} 0.277} & {\color[HTML]{21A0FF} 0.217} \\
657  a woman with short   hair indoors & \checkmark & \checkmark &  & \checkmark & 0.020 & 0.061 & 0.054 \\
658  two or more people   under a tree & \checkmark & \checkmark &  & \checkmark & 0.034 & 0.035 & 0.058 \\
659  a church from the   inside & \checkmark &  &  & \checkmark & 0.342 & {\color[HTML]{21A0FF} 0.188} & 0.255 \\
660  train tracks during   the daytime & \checkmark &  &  &  & 0.524 & {\color[HTML]{21A0FF} 0.361} & {\color[HTML]{21A0FF} 0.211} \\ \bottomrule
\end{tabular}


}
}


\end{table}

==> table/model_adjust_txt_encoder.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tbh!]
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\begin{center}
\scalebox{0.8}{

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{model}} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} & \textbf{Med r} & \multicolumn{1}{c|}{\textbf{mAP}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Text \\ features\end{tabular}}} \\ \hline
W2VV++ & 10.1 & 27.2 & 37.6 & 22 & 0.189 & BoW \\ \hline
W2VV++ & 10.9 & 29.0 & 39.8 & 19 & 0.202 & +W2V \\ \hline
W2VV++ & 11.2 & 29.9 & 40.8 & 18 & 0.207 & +GRU \\ \hline
W2VV++ & 15.1 & 36.0 & 47.4 & 12 & 0.255 & +clip \\ \hline
W2VV++ & 13.9 & 34.9 & 46.0 & 13 & 0.243 & +BERT \\ \hline
SEA & 10.2 & 27.2 & 37.5 & 22 & 0.190 & BoW \\ \hline
SEA & 11.6 & 30.3 & 41.4 & 17 & 0.211 & +W2V \\ \hline
SEA & 11.9 & 31.0 & 42.2 & 16 & 0.216 & +GRU \\ \hline
SEA & 14.7 & 36.0 & 47.4 & 12 & 0.254 & +clip \\ \hline
SEA & 14.8 & 36.3 & 47.8 & 12 & 0.255 & +BERT \\ \hline
LAFF & 10.5 & 28.1 & 38.7 & 20 & 0.196 & BoW \\ \hline
LAFF & 11.0 & 29.1 & 40.0 & 19 & 0.203 & +W2V \\ \hline
LAFF & 11.4 & 30.1 & 40.9 & 18 & 0.210 & +GRU \\ \hline
LAFF & 16.0 & 37.3 & 48.6 & 11 & 0.266 & +clip \\ \hline
LAFF & 16.0 & 37.2 & 48.6 & 11 & 0.266 & +BERT \\ \hline
\end{tabular}

}
\end{center}
\caption{Retrieval performance comparisons among W2VV++, SEA, and LAFF in different text features on MSR-VTT full split.}
\label{tab:model_adjust_txt_encoder}

\end{table}

==> table/model_adjust_vis_encoder.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tbh!]
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\begin{center}
\scalebox{0.8}{

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{model}} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} & \textbf{Med r} & \multicolumn{1}{c|}{\textbf{mAP}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}video \\ features\end{tabular}}} \\ \hline
W2VV++ & 10.256 & 28.023 & 38.63 & 21 & 0.194 & rx101 \\ \hline
W2VV++ & 11.242 & 29.903 & 40.838 & 18 & 0.207 & +re152 \\ \hline
W2VV++ & 13.264 & 33.527 & 44.856 & 14 & 0.234 & +wsl \\ \hline
W2VV++ & 13.948 & 35.075 & 46.585 & 13 & 0.245 & +clip \\ \hline
W2VV++ & 14.694 & 36.47 & 47.997 & 12 & 0.255 & +ircsn \\ \hline
W2VV++ & 14.607 & 36.41 & 47.724 & 12 & 0.254 & +c3d \\ \hline
W2VV++ & 15.115 & 37.259 & 48.943 & 11 & 0.26 & +tf \\ \hline
W2VV++ & 12.54 & 33.273 & 44.865 & 14 & 0.229 & +x3d \\ \hline
SEA & 11.436 & 30.371 & 41.431 & 17 & 0.211 & rx101 \\ \hline
SEA & 11.906 & 31.01 & 42.176 & 16 & 0.216 & +re152 \\ \hline
SEA & 13.851 & 35.074 & 46.717 & 12 & 0.244 & +wsl \\ \hline
SEA & 14.711 & 36.973 & 48.813 & 11 & 0.257 & +clip \\ \hline
SEA & 15.672 & 38.346 & 50.41 & 10 & 0.268 & +ircsn \\ \hline
SEA & 15.266 & 37.729 & 49.592 & 11 & 0.263 & +c3d \\ \hline
SEA & 15.022 & 37.637 & 49.659 & 11 & 0.262 & +tf \\ \hline
SEA & 15.321 & 38.189 & 50.211 & 10 & 0.265 & +x3d \\ \hline
LAFF & 10.987 & 28.946 & 39.734 & 19 & 0.203 & rx101 \\ \hline
LAFF & 11.398 & 30.14 & 40.873 & 18 & 0.21 & +re152 \\ \hline
LAFF & 13.732 & 34.42 & 45.774 & 13 & 0.241 & +wsl \\ \hline
LAFF & 16.833 & 39.819 & 51.729 & 10 & 0.281 & +clip \\ \hline
LAFF & 17.01 & 40.316 & 51.998 & 9 & 0.284 & +ircsn \\ \hline
LAFF & 17.117 & 40.278 & 52.406 & 9 & 0.285 & +c3d \\ \hline
LAFF & 16.821 & 40.368 & 52.237 & 9 & 0.283 & +tf \\ \hline
LAFF & 16.724 & 40.386 & 52.323 & 9 & 0.283 & +x3d \\ \hline
\end{tabular}

}
\end{center}
\caption{Retrieval performance comparisons among W2VV++, SEA, and LAFF in different video features on MSR-VTT full split. }
\label{tab:model_adjust_vis_encoder}

\end{table}
